SMARTmBOT: A ROS2-based Low-cost and Open-source Mobile Robot Platform

This paper introduces SMARTmBOT, an open-source mobile robot platform based on Robot Operating System 2 (ROS2). The characteristics of the SMARTmBOT, including low-cost, modular-typed, customizable and expandable design, make it an easily achievable and effective robot platform to support broad robotics research and education involving either single-robot or multi-robot systems. The total cost per robot is approximately $210, and most hardware components can be fabricated by a generic 3D printer, hence allowing users to build the robots or replace any broken parts conveniently. The SMARTmBot is also equipped with a rich range of sensors, making it competent for general task scenarios, such as point-to-point navigation and obstacle avoidance. We validated the mobility and function of SMARTmBOT through various robot navigation experiments and applications with tasks including go-to-goal, pure-pursuit, line following, and swarming. All source code necessary for reading sensors, streaming from an embedded camera, and controlling the robot including robot navigation controllers is available through an online repository that can be found at https://github.com/SMARTlab-Purdue/SMARTmBOT.

==> wonse_test <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%            /\             /\            %
%           |`\\_,--="=--,_//`|           %
%           \ ."  :'. .':  ". /           %
%          ==)  _ :  '  : _  (==          %
%            |>/O\   _   /O\<|            %
%            | \-"~` _ `~"-/ |            %
%           >|`===. \_/ .===`|<           %
%     .-"-.   \==='  |  '===/   .-"-.     %
%.---{'. '`}---\,  .-'-.  ,/---{.'. '}---.%
% )  `"---"`     `~-===-~`     `"---"`  ( %
%(  Ruiqi, please update this section.  )%
%'---------------------------------------'%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
